Item Graph Convolution Collaborative Filtering for Inductive Recommendations

Graph Convolutional Networks (GCN) have been recently employed as core component in the construction of recommender system algorithms, interpreting user-item interactions as the edges of a bipartite graph. However, in the absence of side information, the majority of existing models adopt an approach of randomly initialising the user embeddings and optimising them throughout the training process. This strategy makes these algorithms inherently transductive, curtailing their ability to generate predictions for users that were unseen at training time. To address this issue, we propose a convolution-based algorithm, which is inductive from the user perspective, while at the same time, depending only on implicit user-item interaction data. We propose the construction of an item-item graph through a weighted projection of the bipartite interaction network and to employ convolution to inject higher order associations into item embeddings, while constructing user representations as weighted sums of the items with which they have interacted. Despite not training individual embeddings for each user our approach achieves state of-the-art recommendation performance with respect to transductive baselines on four real-world datasets, showing at the same time robust inductive performance.

==> tables/datasets_stats.tex <==
\begin{table}
\caption{Dataset statistics}
\centering
\label{table:dataset statistics} 
\begin{tabular}{ccccc}
\toprule 
Dataset & Users & Items & Interactions & Density\\
\midrule
LastFM&
1\,797 & 1\,507 & 62\,376 & 2.30\% \\

Movielens1M&
6\,033 & 3\,123 & 834\,449 & 4.43\% \\

AmazonElectronics&
13\,455 & 8\,360 & 234\,521 & 0.21\% \\

Gowalla&
29\,858 & 40\,988 & 1\,027\,464 & 0.08\% \\
\bottomrule 
\end{tabular} 
\label{table:dataset_stats}
\end{table}

==> tex_figures/1fig_performance_upl.tex <==
 \begin{figure}
    \centering
    \includegraphics[width=\textwidth, keepaspectratio]{images/1fig_User_Profile_Performance.pdf}
    
     \caption{Performance comparison over different cluster of users, grouped based on the user-profile length for the four studied datasets. On the background the histogram shows the number of users in each cluster while the foreground lines report the performance on NDCG@20.}
    \label{fig:Performance_upl}   
\end{figure}
 


==> tex_figures/ablation-cdepth.tex <==
\begin{figure}
    \newcommand{\subfwidth}{0.8\textwidth}
    \centering
    \begin{subfigure}{0.49\textwidth}
        \centering
        \caption{LastFM}
        \includegraphics[width=\subfwidth, keepaspectratio]{images/lastfm_dat_ablation_convolution_depth_NDCG@20.pdf}
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \centering
        \caption{Movielens1M}
        \includegraphics[width=\subfwidth, keepaspectratio]{images/ml1m_dat_ablation_convolution_depth_NDCG@20.pdf}
    \end{subfigure}\\
    \begin{subfigure}{0.49\textwidth}
        \centering
        \caption{Amazon Electronics}
        \includegraphics[width=\subfwidth, keepaspectratio]{images/Amaz_dat_ablation_convolution_depth_NDCG@20.pdf}
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \centering
        \caption{Gowalla}
        \includegraphics[width=\subfwidth, keepaspectratio]{images/gowalla_dat_ablation_convolution_depth_NDCG@20.pdf}
    \end{subfigure}
     \caption{Ablation study: Effect of the Convolution depth parameter on the algorithm performance. On the horizontal axis is reported the value of the hyperparameters while on the vertical axis is reported the NDCG@20.}
    \label{fig:ablation_cdepth}
\end{figure}

==> tex_figures/ablation-dropout.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}{0.25\columnwidth}
        \caption{LastFM}
        \includegraphics[width=\columnwidth, keepaspectratio]{images/lastfm_dat_ablation_dropout_NDCG@20.pdf}
    \end{subfigure}
    \begin{subfigure}{0.25\columnwidth}
        \caption{Ml1M}
        \includegraphics[width=\columnwidth, keepaspectratio]{images/ml1m_dat_ablation_dropout_NDCG@20.pdf}
    \end{subfigure}\\
    \begin{subfigure}{0.25\columnwidth}
        \caption{AE}
        \includegraphics[width=\columnwidth, keepaspectratio]{images/Amaz_dat_ablation_dropout_NDCG@20.pdf}
    \end{subfigure}
    \begin{subfigure}{0.25\columnwidth}
        \caption{Gowalla}
        \includegraphics[width=\columnwidth, keepaspectratio]{images/gowalla_dat_ablation_dropout_NDCG@20.pdf}
    \end{subfigure}
     \caption{Ablation study: Effect of the dropout mechanisms on the algorithm performance. On the horizontal axis is reported the dropout rate while on the vertical axis is reported the NDCG@20.}
    \label{fig:ablation_dropout}
\end{figure*}

==> tex_figures/ablation-topk.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}{0.25\columnwidth}
        \caption{LastFM}
        \includegraphics[width=\columnwidth, keepaspectratio]{images/lastfm_dat_ablation_topk_NDCG@20.pdf}
    \end{subfigure}
    \begin{subfigure}{0.25\columnwidth}
        \caption{Movielens1M}
        \includegraphics[width=\columnwidth, keepaspectratio]{images/ml1m_dat_ablation_topk_NDCG@20.pdf}
    \end{subfigure}\\
    \begin{subfigure}{0.25\columnwidth}
        \caption{Amazon Electronics}
        \includegraphics[width=\columnwidth, keepaspectratio]{images/Amaz_dat_ablation_topk_NDCG@20.pdf}
    \end{subfigure}
    \begin{subfigure}{0.25\columnwidth}
        \caption{Gowalla}
        \includegraphics[width=\columnwidth, keepaspectratio]{images/gowalla_dat_ablation_topk_NDCG@20.pdf}
    \end{subfigure}
     \caption{Effect of the top-K preprocessing step on the algorithm performance and training time. On the background the histogram shows the training time, while the line report the algorithm performance on NDCG@20.}
    \label{fig:ablation_top-k}
\end{figure*}

==> tex_figures/algorithm_pseudocode.tex <==
\begin{algorithm}
\caption{\label{alg:gccf} IGCCF}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\
%\Input{Item embeddings $\textbf{X}_{I\times F}$}\
\Input{Propagation matrix $\textbf{P}_{I\times I}$}\
\Input{User interaction matrix $\tilde{\textbf{R}}_{U\times I}$}\
\Input{Convolution depth $k$}\
\Input{User-profile dropout $p$}\
\Output{Item embeddings $\textbf{X}_{I\times F}$}\

$\textbf{X} \leftarrow $ initialize(\textbf{X}) (${I\times F}$ item embeddings)\;
\While{not converged}{
$B \leftarrow \{(u, i^+, i^-)\}$ sample mini-batch of triplets\;

\For{$j = 1,\dots, k$}{
    $\textbf{X} \leftarrow \textbf{P}\textbf{X}$
}
$\tilde{\textbf{R}} \leftarrow$  user-profile dropout ($\tilde{\textbf{R}}$, $p$)\;

$\textbf{U} \leftarrow \tilde{\textbf{R}}\textbf{X}$\;
$\nabla L(\textbf{X} )\leftarrow$ compute gradients $L_{BPR}(\textbf{X}$,$\textbf{U}$,$B$)\;
$\textbf{X} \leftarrow$ apply gradients($\nabla L(\textbf{X})$)
}
\end{algorithm}

==> tex_figures/inductive-performance.tex <==
\begin{figure*}[!t]
    \centering
    %\captionsetup[subfigure]{labelformat=empty}
    \begin{subfigure}{0.25\columnwidth}
        \caption{LastFM}
        \includegraphics[width=\columnwidth, keepaspectratio]{images/lastfm_dat_unseen_users_performance@20.pdf}
    \end{subfigure}
    \begin{subfigure}{0.25\columnwidth}
        \caption{Movielens1M}
        \includegraphics[width=\columnwidth, keepaspectratio]{images/ml1m_dat_unseen_users_performance@20.pdf}
    \end{subfigure}\\
    \begin{subfigure}{0.25\columnwidth}
        \caption{Amazon Electronics}
        \includegraphics[width=\columnwidth, keepaspectratio]{images/Amaz_dat_unseen_users_performance@20.pdf}
    \end{subfigure}
    \begin{subfigure}{0.25\columnwidth}
        \caption{Gowalla}
        \includegraphics[width=\columnwidth, keepaspectratio]{images/gowalla_dat_unseen_users_performance@20.pdf}
    \end{subfigure}
     \caption{For each dataset we vary the percentage of users in the training data, and evaluate the performance of IGCCF on both \textit{seen} and \textit{unseen} users. We perform the experiments $5$ different times reporting the average NDCG@20 performance along with the standard deviation.}
%     On the horizontal axis is reported the percentage of users used in the training data while on the vertical axis is reported the NDCG@20}
    \label{fig:Inductive_performance}
\end{figure*}

==> tex_figures/performance-upl.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}{0.25\columnwidth}
        \caption{LastFM}
        \includegraphics[width=\columnwidth, keepaspectratio]{images/lastfm_dat_NDCG@20_User_Profile_length_performance.pdf}
    \end{subfigure}
    \begin{subfigure}{0.25\columnwidth}
        \caption{Movielens1M}
        \includegraphics[width=\columnwidth, keepaspectratio]{images/ml1m_dat_NDCG@20_User_Profile_length_performance.pdf}
    \end{subfigure}\\
    \begin{subfigure}{0.25\columnwidth}
        \caption{Amazon Electronics}
        \includegraphics[width=\columnwidth, keepaspectratio]{images/Amaz_dat_NDCG@20_User_Profile_length_performance.pdf}
    \end{subfigure}
    \begin{subfigure}{0.25\columnwidth}
        \caption{Gowalla}
        \includegraphics[width=\columnwidth, keepaspectratio]{images/gowalla_dat_NDCG@20_User_Profile_length_performance.pdf}
    \end{subfigure}
     \caption{Performance comparison over different cluster of users, grouped based on the user-profile length for the four studied datasets. On the background the histogram shows the number of users in each cluster while the foreground lines report the performance on NDCG@20.}
    \label{fig:Performance_upl}
\end{figure*}
